Real-time Nonlinear Model Predictive Control using One-step Optimizations and Reachable Sets

Model predictive control allows solving complex control tasks with control and state constraints. However, an optimal control problem must be solved in real-time to predict the future system behavior, which is hardly possible on embedded hardware. To solve this problem, this paper proposes to compute a sequence of one-step optimizations aided by pre-computed inner approximations of reachable sets rather than solving the full-horizon optimal control problem at once. This feature can be used to virtually predict the future system behavior with a low computational footprint. Proofs for recursive feasibility and for the sufficient conditions for asymptotic stability under mild assumptions are given. The presented approach is demonstrated in simulation for functional verification.

==> BasicMPC.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\figW,
height=\figH,
at={(0\figW,0\figH)},
scale only axis,
xmin=0,
xmax=10,
xtick={0,1,2,10},
xticklabels={{$\text{t}_\text{0}$},{$\text{t}_{\text{0+1}}$},{$\text{t}_{\text{0+2}}$},{$\text{t}_{\text{0+T}}$}},
ymin=-2,
ymax=1,
ytick={-1.37561739049018,-0.4},
yticklabels={{$\text{u}_\text{P}\text{(t)}$},{$\text{x}_\text{P}\text{(t)}$}},
axis background/.style={fill=white}
]
\addplot [color=black, line width=1.0pt, forget plot]
  table[row sep=crcr]{%
0	-0.4\\
0.0999999999999996	-0.379039656019799\\
0.300000000000001	-0.332780868213289\\
0.699999999999999	-0.235828864871536\\
0.9	-0.190260541533599\\
1.1	-0.148710821882439\\
1.2	-0.129711559247312\\
1.3	-0.111978919324594\\
1.4	-0.0955438869323508\\
1.5	-0.0804165122119276\\
1.6	-0.0665889381037736\\
1.7	-0.0540381774452641\\
1.8	-0.0427286538974787\\
2	-0.0236417495758037\\
2.2	-0.00887454176500313\\
2.4	0.00210146453298776\\
2.6	0.00984415047673792\\
2.8	0.0149063679220749\\
3	0.0178112309500271\\
3.3	0.019151704293936\\
3.6	0.0180680360117798\\
4.1	0.0136418616119283\\
4.9	0.00590273209379433\\
5.6	0.00201911361212836\\
6.3	-0.000221035133865399\\
7.3	-0.000848044823396066\\
10	0.000157211228533072\\
};
\addplot [color=black, line width=1.0pt, draw=none, mark=asterisk, mark options={solid, black}, forget plot]
  table[row sep=crcr]{%
0	-0.4\\
1	-0.1689214923733\\
2	-0.0236417495758037\\
3	0.0178112309500271\\
4	0.0146545941916632\\
6	0.000481940861085661\\
7	-0.000844063994176025\\
8	-0.000621896556786794\\
9	-0.00022591970231467\\
10	0.000157211228533072\\
};
\addplot [color=black, line width=1.0pt, draw=none, mark=asterisk, mark options={solid, black}, forget plot]
  table[row sep=crcr]{%
5	0.00511670042713774\\
};
\addplot[const plot, color=black, line width=1.0pt, forget plot] table[row sep=crcr] {%
0	-1.37561739049018\\
1	-1.47345239364971\\
2	-1.20331183729943\\
3	-1.02872912514167\\
4	-0.978659223391906\\
6	-0.992891015582645\\
7	-0.999417492275969\\
8	-1.00097910397967\\
9	-1.00060188583461\\
10	-1\\
};
\addplot [color=white!70!black, dashed, forget plot]
  table[row sep=crcr]{%
1	-2\\
1	1\\
};
\addplot [color=white!70!black, dashed, forget plot]
  table[row sep=crcr]{%
2	-2\\
2	1\\
};
\addplot [color=white!70!black, dashed, forget plot]
  table[row sep=crcr]{%
3	-2\\
3	1\\
};
\addplot [color=white!70!black, dashed, forget plot]
  table[row sep=crcr]{%
4	-2\\
4	1\\
};
\addplot [color=white!70!black, dashed, forget plot]
  table[row sep=crcr]{%
5	-2\\
5	1\\
};
\addplot [color=white!70!black, dashed, forget plot]
  table[row sep=crcr]{%
6	-2\\
6	1\\
};
\addplot [color=white!70!black, dashed, forget plot]
  table[row sep=crcr]{%
7	-2\\
7	1\\
};
\addplot [color=white!70!black, dashed, forget plot]
  table[row sep=crcr]{%
8	-2\\
8	1\\
};
\addplot [color=white!70!black, dashed, forget plot]
  table[row sep=crcr]{%
9	-2\\
9	1\\
};
\end{axis}
\end{tikzpicture}%
